Succinct Oblivious Tensor Evaluation and Applications: Adaptively-Secure Laconic Function Evaluation and Trapdoor Hashing for All Circuits

We propose the notion of succinct oblivious tensor evaluation (OTE), where two parties compute an additive secret sharing of a tensor product of two vectors $\mathbf{x} \otimes \mathbf{y}$, exchanging two simultaneous messages. Crucially, the size of both messages and of the CRS is independent of the dimension of $\mathbf{x}$. We present a construction of OTE with optimal complexity from the standard learning with errors (LWE) problem. Then we show how this new technical tool enables a host of cryptographic primitives, all with security reducible to LWE, such as: * Adaptively secure laconic function evaluation for depth-$D$ functions $f:\{0, 1\}^m\rightarrow\{0, 1\}^\ell$ with communication $m+\ell+D\cdot \mathrm{poly}(\lambda)$. * A trapdoor hash function for all functions. * An (optimally) succinct homomorphic secret sharing for all functions. * A rate-$1/2$ laconic oblivious transfer for batch messages, which is best possible. In particular, we obtain the first laconic function evaluation scheme that is adaptively secure from the standard LWE assumption, improving upon Quach, Wee, and Wichs (FOCS 2018). As a key technical ingredient, we introduce a new notion of \emph{adaptive lattice encodings}, which may be of independent interest.

==> figure.tex <==
\begin{figure*}
    \centering
\begin{tikzpicture}[
  node distance=2cm and 3cm,
  primitive/.style={draw, rounded corners, align=center, font=\small},
  ref/.style={font=\scriptsize, midway, sloped, above},
  ref-nonsloped/.style={font=\scriptsize},
  scale = 0.8
]

% Nodes
\node[primitive] (half) at (-5,0) {Half-Succinct NI-OTE%\\(Section~\ref{sec:halfNIOTE})
};
\node[primitive] (niote) at (0,0) {Succinct NI-OTE%\\(Section~\ref{sec:NIOTE})
};
\node[primitive] (mole) at (0,2) {Succinct NI-MOLE%\\(Section~\ref{sec:MOLE})
};
\node[primitive] (lenc) at (-5,-2) {Adaptive Lattice Encodings%\\(Section~\ref{sec:hom_enc})
};
\node[primitive] (comp) at (2,-2) {Compressed Encodings%\\(Section~\ref{sec:comp_enc})
};
\node[primitive] (LFE) at (2,4) {Laconic Function Evaluation\\ \cite{FOCS:QuaWeeWic18,FOCS:HsiLinLuo23,C:DHMWW24}};
\node[primitive] (RTDH) at (5,2) {Reverse TDH%\\(Section~\ref{sec:rtdh})
};
\node[primitive] (TDH) at (10,3) {Regular TDH};
\node[primitive] (HSS) at (10,2) {Succinct HSS};
\node[primitive] (LOT) at (10,1) {Rate-$1/2$ Laconic OT};
\node[primitive] (wRTDH) at (5.5,0) {Input-Succinct Reverse TDH%\\(Section~\ref{sec:weakTDH})
};
\node[primitive] (mainLFE) at (9,-2) {Rate-1 Adaptively Secure LFE%\\(Section~\ref{sec:mainLFE})
};


% % Arrows
\draw[->] (half) -- (niote);
\draw[->] (niote) -- (mole);
\draw[->] (mole) -- (RTDH);
\draw[->] (LFE) to [bend left=10] node{} (RTDH);
\draw[->] (RTDH) to [bend left=10] node{} (TDH);
\draw[->] (RTDH) -- (HSS);
\draw[->] (RTDH) to [bend right=10] node{} (LOT);
\draw[->] (niote) to [bend right=20] node{} (comp);
\draw[->] (lenc) -- (comp);
\draw[->] (comp) to [bend right=20] node{} (wRTDH);
\draw[->] (mole) to [bend left=20] node{} (wRTDH);
\draw[->] (wRTDH) to [bend left=20] node{} (mainLFE);


\end{tikzpicture}
\caption{A schematic representation of our results, and a summary of the implications to different cryptographic primitives.}\label{fig:diagram}
\end{figure*}

==> macros.tex <==
% !TEX root = main.tex
% !TEX spellcheck = en-US

\mathchardef\mhyphen="2D

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% ENVIRONMENTS %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{observation}{Observation}
\newtheorem{assumption}{Assumption}

% markup:
\newcommand{\markchanged}[1]{{\color{red} #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% MISC NOTATION %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{yuval}[1]{{\color{blue}[Yuval: {#1}]}}

\newcommand{\hek}{\mathsf{pk'}}
\newcommand{\hct}{\mathsf{hct}}
\newcommand{\ek}{\mathsf{ek}}
\newcommand{\ak}{\mathsf{ak}}
\newcommand{\mek}{\mathsf{mek}}
\newcommand{\mhk}{\mathsf{mhk}}
\newcommand{\td}{\mathsf{td}}
\newcommand{\Auth}{\mathsf{Auth}}
\newcommand{\RFHE}{\mathsf{R1FHE}}
\newcommand{\E}{\mathsf{E}}

\newcommand{\LFE}{\mathsf{LFE}}
\newcommand{\MOLE}{\mathsf{MOLE}}

\newcommand{\etal}{\emph{et al.}\xspace}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\tuple}[1]{(#1)}
\newcommand{\getsr}{\overset{\raisebox{-1pt}{$\scriptscriptstyle \$$}}{\gets}}
\newcommand{\sample}{\getsr}
\newcommand{\compindist}{\approx_{\rm c}}
\newcommand{\statindist}{\approx_{\rm s}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Permute}{\mathsf{Permute}}
\newcommand{\Sym}{\mathsf{Sym}}
\newcommand{\Explain}{\mathsf{Explain}}
\newcommand{\Pre}{\mathsf{Pre}}
\newcommand{\Post}{\mathsf{Post}}
\newcommand{\BOTE}{\mathsf{hOTE}}
\newcommand{\AOTE}{\mathsf{AC\text{-}OTE}}
\newcommand{\AMOLE}{\mathsf{AC\text{-}MOLE}}
\newcommand{\OTE}{\mathsf{OTE}}
\newcommand{\GSW}{\mathsf{GSW}}

% Number sets
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\LWE}{\mathsf{LWE}}
\newcommand{\Reconstruct}{\mathsf{Recover}}
\newcommand{\Inj}{\mathsf{Inj}}
\newcommand{\Plant}{\mathsf{Plant}}
\newcommand{\Subgraph}{\mathsf{Subgraph}}
\newcommand{\Randomise}{\mathsf{Cut}}
\newcommand{\Encode}{\mathsf{Encode}}

% Polynomial/negligible functions
\newcommand{\PRP}{\mathsf{PRP}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\polylog}{\mathsf{polylog}}
\newcommand{\negl}{\mathsf{negl}}
\newcommand{\nonotice}{\mathsf{non\text{-}notic}}

\renewcommand{\sec}{\ensuremath{\lambda}}
\newcommand{\secpar}{\sec}
\newcommand{\ssec}{\kappa}
\newcommand{\bit}{\{0,1\}}
\newcommand{\Prob}{\mathbb{P}} % probability measure
\newcommand{\circuit}{\mathsf{Cr}}

% Indexing
\newcommand{\ith}{^{(i)}}
\newcommand{\ijth}{^{(i_j)}}
\newcommand{\iiotath}{^{(i_\iota)}}
\newcommand{\jth}{^{(j)}}
\newcommand{\zth}{^{(0)}}
\newcommand{\betath}{^{(\beta)}}
\newcommand{\fst}{^{(1)}}
\newcommand{\snd}{^{(2)}}
\newcommand{\Qth}{^{(Q)}}
\newcommand{\mth}{^{(m)}}
\newcommand{\rhoth}{^{(\rho)}}

% Ordering
%\newcommand{\lex}{\ensuremath{\text{lex}}} % lexographical order
\newcommand{\lexe}{\ensuremath{\le_\text{lex}}} % lexographical order
\newcommand{\glexe}{\ensuremath{\ge_\text{lex}}} % lexographical order
\newcommand{\glex}{\ensuremath{>_\text{lex}}} % lexographical order

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% CRYPTO PRIMITIVES %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\DS}{\mathsf{DS}} % distributed sampler
\newcommand{\US}{\mathsf{US}} % universal sampler
\newcommand{\DUS}{\mathsf{DUS}} % distributed universal sampler
\newcommand{\OTUS}{\mathsf{OTUS}} % one-time universal sampler
\newcommand{\SSB}{\mathsf{Hash}} % somewhere statistically binding hash function
\newcommand{\HE}{\mathsf{HE}} % homomorphic encryption
%\newcommand{\PRF}{\ensuremath{F}}
\newcommand{\PPRF}{\ensuremath{F}}
\newcommand{\PRG}{\mathsf{PRG}}
\newcommand{\lex}{<_\mathsf{lex}}
\newcommand{\NIZK}{\mathsf{NIZK'}}
\newcommand{\SOTS}{\mathsf{SOTS}}
\newcommand{\LOWF}{\mathsf{CLOWF}}
\newcommand{\Derive}{\mathsf{Derive}}
\newcommand{\Project}{\mathsf{Project}}
\newcommand{\Progr}{\mathsf{Prog}}
\newcommand{\vk}{\mathsf{vk}}
\newcommand{\Sign}{\mathsf{Sign}}
\newcommand{\KE}{\mathsf{Ex}}
\newcommand{\DDH}{\mathsf{DDH}}
\newcommand{\PCG}{{\mathsf{PCG}}}
\newcommand{\PCF}{{\mathsf{PCF}}}
\newcommand{\pkPCFS}{{\mathsf{pkPCFS}}}
\newcommand{\pkPCF}{{\mathsf{pkPCF}}}
\newcommand{\PKE}{\mathsf{PKE}}
\newcommand{\MHE}{\mathsf{pMHE}}
\newcommand{\ELF}{\mathsf{ELF}}
\newcommand{\mkFHE}{\mathsf{mkFHE}}
\newcommand{\Commit}{\mathsf{Commit}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\Trunc}{\mathsf{Trunc}}
\newcommand{\ct}{\mathsf{ct}}
\newcommand{\NIWI}{\mathsf{NIWI}}
\newcommand{\chk}{\mathsf{Check}}
\newcommand{\lab}{\mathsf{tag}}
\newcommand{\Val}{\mathsf{Val}}
\newcommand{\diO}{\mathsf{diO}}
\newcommand{\Samp}{\mathsf{Samp}}
\newcommand{\aux}{\mathsf{aux}}
\newcommand{\ext}{\mathsf{sk}}
\newcommand{\Trap}{\mathsf{Trap}}
\newcommand{\VPFS}{\mathsf{VPFE}}
\newcommand{\AClass}{\mathsf{AClass}}
\newcommand{\EClass}{\mathsf{EClass}}
\newcommand{\Advantage}{\mathsf{Adv}}
\newcommand{\chall}{\mathsf{Ch}}
\newcommand{\tchall}{\mathsf{Ch}}
\newcommand{\COWF}{\mathsf{COWF}}
\newcommand{\game}{\mathcal{G}}
%\newcommand{\Env}{\mathcal{E}}
\newcommand{\ENIZK}{\mathsf{NIZK}}
\newcommand{\Trapdoor}{\mathsf{Trap}}
\newcommand{\Lossy}{\mathsf{Lossy}}
\newcommand{\nonegl}{\mathsf{nonegl}}
\newcommand{\Supp}{\mathsf{Supp}}
%\newcommand{\Trunc}{\mathsf{Trunc}}
\newcommand{\DI}{\mathsf{DI}}
\newcommand{\Bdv}{\mathcal{B}}
% Protocols
\newcommand{\Prot}[1]{\ensuremath{\Pi_{\mathsf{#1}}}}

\newcommand{\PDUS}{\Prot{DUS}}
\newcommand{\PDS}{\Prot{DS}}

% Functionalities
\newcommand{\Func}[1]{\ensuremath{\mathcal{F}_{\mathsf{#1}}}}
\newcommand{\FDUSsemimal}{\ensuremath{\Func{DUS}^{\mathsf{semi\text{-}mal}}}}
\newcommand{\FDUSact}{\ensuremath{\Func{DUS}^{\mathsf{active}}}}

% Programs
\newcommand{\Prog}[1]{\ensuremath{\mathcal{P}_{\mathsf{#1}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% PARTIES %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Env}{\mathcal{Z}}
\newcommand{\Sim}{\mathsf{Sim}}
\newcommand{\Adv}{\mathcal{A}}
\newcommand{\AdvB}{\mathcal{B}}
\newcommand{\Chal}{\mathcal{C}}
\newcommand{\Party}{\ensuremath{P}}
\newcommand{\RMS}{\mathsf{RMS}}
\newcommand{\RTDH}{\mathsf{RTDH}}
\newcommand{\BV}{\mathsf{GSW}}
\newcommand{\Compress}{\mathsf{Compress}}
\newcommand{\ck}{\mathsf{ck}}
% # parties; party index
\newcommand{\pts}{\ensuremath{n}} % number of parties
\newcommand{\pix}{\ensuremath{i}} % party idx
\newcommand{\pixh}{\ensuremath{h}} % honest party idx
\newcommand{\pixo}{\ensuremath{j}} % other party idx
\newcommand{\pixoo}{\ensuremath{l}} % other other party idx

\newcommand{\corset}{\ensuremath{C}}
\newcommand{\honset}{\ensuremath{H}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% ALGORITHMS %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\algofont}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\hash}{\algofont{H}}
\newcommand{\tpk}{{\algofont{tpk}}}
\newcommand{\Enc}{{\algofont{Enc}}}
\newcommand{\Dec}{{\algofont{Dec}}}
\newcommand{\Fin}{{\algofont{Fin}}}
\newcommand{\Part}{{\algofont{Part}}}
\newcommand{\Peval}{\algofont{PrivEval}}

\newcommand{\Sample}{{\algofont{Sample}}}
\newcommand{\Correlation}{{\algofont{Correlation}}}
\newcommand{\RSample}{{\algofont{RSample}}}

\newcommand{\Setup}{{\algofont{Setup}}}
\newcommand{\Gen}{{\algofont{Gen}}}
\newcommand{\Share}{{\algofont{Share}}}
\newcommand{\Eval}{\hyperref[alg:eval]{\algofont{Eval}}\xspace}
\newcommand{\FullEval}{\hyperref[alg:fulleval]{\algofont{FullEval}}\xspace}
\newcommand{\Hash}{{\algofont{Hash}}}

\newcommand{\SendMsg}{{\algofont{SendMsg}}}
\newcommand{\GetOutput}{{\algofont{Output}}}
\newcommand{\ARSendMsg}{{\algofont{ARMsg}}}
\newcommand{\ARGetOutput}{{\algofont{AROutput}}}

% Distributed Sampler Ideal Functionality:
\newcommand{\Init}{\algofont{Init}}
\newcommand{\Query}{\algofont{Query}}
\newcommand{\Choice}{\algofont{Choice}}
\newcommand{\Output}{\algofont{Output}}
\newcommand{\Abort}{\algofont{Abort}}

% SSB:
\newcommand{\Open}{\algofont{Open}}
\newcommand{\Verify}{\algofont{Verify}}
\newcommand{\SSBhash}{\SSB.\Hash}

% Multi-key FHE:
\newcommand{\Expand}{\algofont{Expand}}
\newcommand{\PDec}{\algofont{PDec}}
\newcommand{\FDec}{\algofont{FinDec}}
\newcommand{\Simulate}{\algofont{Sim}}
\newcommand{\rel}{\mathcal{R}}

% iO:
\newcommand{\iO}{\algofont{iO}}

% PPRF:
\newcommand{\Punct}{\algofont{Punct}}

% RO:
\newcommand{\RO}{\mathcal{H}}

% NIZK:
\newcommand{\Prove}{\algofont{Prove}}
\newcommand{\Extract}{\algofont{Extract}}

% Universal sampler:
\newcommand{\Simgen}{\algofont{SimGen}}
\newcommand{\SimRO}{\algofont{SimRO}}
\newcommand{\SO}{\mathcal{O}} % sampling oracle

%Garbled Circuits:
\newcommand{\Garble}{\algofont{Garble}}
\newcommand{\GC}{\algofont{GC}}
\newcommand{\EP}{\algofont{EP}}
\newcommand{\EProg}{\algofont{EProg}}
\newcommand{\DP}{\algofont{DP}}
\newcommand{\DProg}{\algofont{DProg}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% OBJECTS %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\advrand}{\ensuremath{\rho}} % random tapes of parties
\newcommand{\params}{\ensuremath{\mathsf{params}}}

% Distributed Sampler:
\newcommand{\dist}{\ensuremath{\mathcal{D}}}
\newcommand{\rand}{\ensuremath{r}} % randomness used for algorithms
\newcommand{\orand}{\ensuremath{w}} % other randomness used for algorithms
\newcommand{\randseed}{\ensuremath{s}} % randomness used to produce the random sample
\newcommand{\rands}{\ensuremath{R}} % random sample from the distribution
\newcommand{\sampler}{\ensuremath{U}}
\newcommand{\asampler}{\ensuremath{Z}}

% Distributed Universal Samplers
\newcommand{\dsize}{\ensuremath{\ell}} % bit length description distribution
\newcommand{\rsize}{\ensuremath{r}} % bit length randomness input in distribution
\newcommand{\osize}{\ensuremath{t}} % bit length output distribution

% Distributed Sampler Ideal Functionality:
\newcommand{\qset}{\ensuremath{Q}}
\newcommand{\id}{\ensuremath{\mathbf{I}}}
\newcommand{\mpk}{\mathsf{mpk}}
\newcommand{\msk}{\mathsf{msk}}
\newcommand{\IBE}{\mathsf{IBE}}
\newcommand{\OWF}{\mathsf{OWF}}
\newcommand{\Com}{\mathsf{Com}}
\newcommand{\CCA}{\mathsf{CCA}}
\newcommand{\KH}{\mathsf{KHash}}
\newcommand{\sid}{\mathsf{sid}}
\newcommand{\ID}{\mathsf{ID}}
\newcommand{\tgame}{\mathcal{G}}
%\newcommand{\tag}{\mathsf{tag}}
%\newcommand{\Check}{\mathsf{Check}}
\newcommand{\shannon}{\mathsf{H}}
% Common MISC:
\newcommand{\crs}{\mathsf{crs}}
\newcommand{\urs}{\mathsf{urs}}
\newcommand{\pk}{{\mathsf{pk}}}
\newcommand{\sk}{{\mathsf{sk}}}
\newcommand{\msg}{\ensuremath{\mathsf{g}}}
\newcommand{\armsg}{\ensuremath{\mathsf{armsg}}}
\newcommand{\ctext}{\ensuremath{c}}
\newcommand{\key}{\ensuremath{K}}
\newcommand{\okey}{\ensuremath{k}} % other key
\newcommand{\trapdoor}{\ensuremath{\tau}}
\newcommand{\outp}{\ensuremath{\mathsf{res}}}

% Obfuscation
\newcommand{\circuitclass}{\mathcal{L}}  % circuit class
\newcommand{\obfinput}{\mathsf{inp}}  % input size
\newcommand{\obfoutput}{\mathsf{out}} % output size

% PPRF
\newcommand{\outspace}{\mathcal{X}} % output space


% SSB:
\newcommand{\hk}{\ensuremath{\mathsf{hk}}}
\newcommand{\bsize}{\ensuremath{B}} % block size

% Multi-key FHE:
\newcommand{\pdec}{\ensuremath{d}}

% Distributed Sampler Constructions:
\newcommand{\KGP}{\ensuremath{\mathsf{KGP}}} % the key-generation program
\newcommand{\EvP}{\ensuremath{\mathsf{EvP}}} % the evaluation program
\newcommand{\SP}{\ensuremath{\mathsf{S}}}

% Active Compiler
\newcommand{\psample}{\ensuremath{\msg}} % party sample
\newcommand{\ROctext}{\ensuremath{u}} % first part of the oracle response
\newcommand{\ROnonce}{\ensuremath{v}} % second part of the oracle response
\newcommand{\expnonce}{\ensuremath{y}} % expansion of \ROnonce using PPRF
\newcommand{\expexpnonce}{\ensuremath{e}} % double expansion of \ROnonce using PPRF and PRG
\newcommand{\ROplain}{\ensuremath{x}} % decryption of the oracle response
\newcommand{\ssize}{\ensuremath{m}} % size of the sampler share
\newcommand{\ndist}{\ensuremath{\SendMsg}} % n-party distribution

% PCF stuff
\newcommand{\mk}{{\mathsf{mk}}}
\newcommand{\corr}{{\mathcal{C}}}
\newcommand{\Secret}{\algofont{Secret}}
\newcommand{\GRSample}[3]{\mathcal{G}^\text{#1, RSample}_{#2, #3}(\secpar)}
\newcommand{\GCorr}{\mathcal{G}_\text{Corr}(\secpar)}
\newcommand{\GSec}{\mathcal{G}_\text{Sec}^\corset(\secpar)}
\newcommand{\GCorrPCF}{\mathcal{G}_{\text{PCF}\mhyphen\text{Corr}}(\secpar)}
\newcommand{\GSecPCF}{\mathcal{G}_{\text{PCF}\mhyphen\text{Sec}}^{\corset, (\advrand_i)_{i\in\corset}}(\secpar)}
\newcommand{\GSetupCorr}{\mathcal{G}_\text{SetupCorr}(\secpar)}
\newcommand{\GSetupSec}{\mathcal{G}_\text{SetupSec}^{\corset, (\advrand_i)_{i\in\corset}}(\secpar)}
\newcommand{\nsize}{\ensuremath{l}} % nonce size
\newcommand{\nonce}{\ensuremath{x}}
%\newcommand{\nonceset}{\ensuremath{X}}

%pMHE
\newcommand{\GpMHE}{\mathcal{G}_\text{pMHE}^{\corset, \circuit, (x_\pixh)_{\pixh\in\honset}}(\secpar)}

% PCF construction
\newcommand{\CGP}{\ensuremath{\mathsf{CGP}}} % correlation generator program
\newcommand{\PCFcrs}{\ensuremath{S}}

% Access Struct:
\newcommand{\minset}[1]{\ensuremath{\min\left(#1\right)}}
\newcommand{\maxset}[1]{\ensuremath{\max\left(\overline{#1}\right)}}

% NIZK:
\newcommand{\relation}{\ensuremath{\mathcal{R}}}
\newcommand{\statement}{\ensuremath{\phi}}
\newcommand{\witness}{\ensuremath{w}}
\newcommand{\zkproof}{\ensuremath{\pi}}

% Universal sampler
\newcommand{\GUS}{\mathcal{G}_\text{US}(\secpar)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% REFERENCING %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\applab}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
%\renewcommand{\appref}[1]{the full version of this paper}
\newcommand{\lemmaref}[1]{Lemma~\ref{lem:#1}}


\newcommand{\figlab}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
%\renewcommand{\eqref}[1]{(\ref{eq:#1})}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\seclab}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\maybesecref}[1]{\iffull{Section}{Appendix}~\ref{sec:#1}}
\newcommand{\maybesubsecref}[1]{\iffull{Section}{Appendix}~\ref{subsec:#1}}
\newcommand{\protref}[1]{Protocol~\ref{alg:#1}}
\newcommand{\thmlab}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemlab}[1]{\label{lemma:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lemma:#1}}
\newcommand{\deflab}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\asslab}[1]{\label{assumption:#1}}
\newcommand{\assref}[1]{Assumption~\ref{assumption:#1}}
\newcommand{\corlab}[1]{\label{corollary:#1}}
\newcommand{\corref}[1]{Corollary~\ref{corollary:#1}}











\newcommand{\jnote}[1]{{\color{blue}jack: {#1}}}
\newcommand{\ynote}[1]{{\color{red}Yuval: {#1}}}


\newcommand{\fcoin}{\ensuremath{\Func{\hyperref[func:coin]{Coin}}^n}\xspace}
\newcommand{\fcoinsimple}{\ensuremath{\Func{\hyperref[func:coinsimple]{Coin}}^n}\xspace}
\newcommand{\fcoinm}{\ensuremath{\Func{\hyperref[func:coin]{Coin}}^m}\xspace}
\newcommand{\fcoinsimplem}{\ensuremath{\Func{\hyperref[func:coinsimple]{Coin}}^m}\xspace}
\newcommand{\fcoinsec}{\ensuremath{\Func{\hyperref[func:coin]{Coin}}^\sec}\xspace}
\newcommand{\fcoinia}{\ensuremath{\Func{\hyperref[func:coin_ia]{Coin+IA}}^m}\xspace}
\newcommand{\fhssetup}{\ensuremath{\Func{\hyperref[func:HSSetup]{HS\text{-}Setup}}}\xspace}
\newcommand{\fdist}{\ensuremath{\Func{\hyperref[func:samplingfunc]{\dist}}}\xspace}
\newcommand{\pctia}{\ensuremath{\Prot{\hyperref[func:samplingfunc]{CT\text{-}IA}}}\xspace}
\newcommand{\token}[1]{\ensuremath{\texttt{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%llncs things%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifdefined\isllncs\else
\newcommand\bbbone{1}
\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Tableofcontents}{
\ifdefined\isllncs
\ifdraft{
    \clearpage
    \setcounter{tocdepth}{2}
    \tableofcontents
    \clearpage
    \pagebreak
    \thispagestyle{empty}
}{}
\else
    \thispagestyle{empty}
    \pagenumbering{gobble}
    \clearpage
    \setcounter{tocdepth}{2}
    \tableofcontents
    \thispagestyle{empty}
    \clearpage
    \pagenumbering{arabic}
\fi
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Cref issues
%make all reference start with uppercase
%\renewcommand{\cref}{\Cref}

\ifdefined\isllncs
    \newtheoremstyle{ihatelncs}
    {\topsep}                % Space above
    {}                % Space below
    {\itshape}        % Theorem body font % (default is "\upshape")
    {}                % Indent amount
    {}       % Theorem head font % (default is \mdseries)
    {}               % Punctuation after theorem head % default: no punctuation
    { }               % Space after theorem head
    {{\bfseries \thmname{#1}\thmnumber{ #2}.}\thmnote{ (#3){\bfseries.}}~}                % Theorem head spec
    \theoremstyle{ihatelncs}

    \newtheorem{theoreml}{Theorem}[section]
    \renewenvironment{theorem}{\begin{theoreml}}{\end{theoreml}}

    \newtheorem{lemmal}[theoreml]{Lemma}
    \renewenvironment{lemma}{\begin{lemmal}}{\end{lemmal}}

    \newtheorem{claiml}[theoreml]{Claim}
    \renewenvironment{claim}{\begin{claiml}}{\end{claiml}}

    \newtheorem{corollaryl}[theoreml]{Corollary}
    \renewenvironment{corollary}{\begin{corollaryl}}{\end{corollaryl}}

    \newtheorem{propositionl}[theoreml]{Proposition}
    \renewenvironment{proposition}{\begin{propositionl}}{\end{propositionl}}

    \newtheorem{conjecturel}[theoreml]{Conjecture}
    \renewenvironment{conjecture}{\begin{conjecturel}}{\end{conjecturel}}

    \newtheorem{definitionl}[theoreml]{Definition}
    \renewenvironment{definition}{\begin{definitionl}}{\end{definitionl}}

    \newtheorem{factl}[theoreml]{Fact}
    \newenvironment{fact}{\begin{factl}}{\end{factl}}

    \newtheorem{remarkl}[theoreml]{Remark}
    \renewenvironment{remark}{\begin{remarkl}}{\end{remarkl}}

    \newtheorem{examplel}[theoreml]{Example}
    \renewenvironment{example}{\begin{examplel}}{\end{examplel}}

    \newaliascnt{boxctr}{theoreml}
    \renewcommand\thetheoreml{\thesection.\arabic{theoreml}}
    \makeatletter
    \let\c@table\c@theoreml
    \makeatother
    \renewcommand\thetable{\thesection.\arabic{theoreml}}
\else
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{claim}[theorem]{Claim}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{conjecture}[theorem]{Conjecture}
    \newtheorem{definition}[theorem]{Definition}
    \newtheorem{fact}[theorem]{Fact}
    \newtheorem{remark}[theorem]{Remark}
    \newtheorem{example}[theorem]{Example}
    \newaliascnt{boxctr}{theorem}
    \makeatletter
    \let\c@table\c@theorem
    \makeatother
    \renewcommand\thetable{\thesection.\arabic{theorem}}
\fi

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}
\newreptheorem{corollary}{Corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%===========Hybrid/Proof stuff================
\makeatletter
\newcommand*\ifcounter[1]{%
  \ifcsname c@#1\endcsname
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\makeatother

\newcounter{realfirsthybrid}
\newcounter{realhybrids}
\setcounter{realhybrids}{1}
\newcounter{realprevhybrid}
\setcounter{realprevhybrid}{0}
\newcounter{hybrids}
\newcounter{prevhybrid}
\newcommand{\inithybrids}[1]{\setcounter{hybrids}{#1}\setcounter{prevhybrid}{#1-1}}
\newcommand{\targetthishybrid}[1]{\setcounter{hybrids}{\arabic{hybrids}-1}\refstepcounter{hybrids}\label{#1}\setcounter{realhybrids}{\arabic{realhybrids}-1}\refstepcounter{realhybrids}\label{real#1}}
\newcommandx{\linkthishybrid}[1][1={}]{\phantomsection\stepcounter{realprevhybrid}\refstepcounter{realhybrids}\setcounter{realfirsthybrid}{\arabic{realhybrids}}\label{hybauto:\arabic{realhybrids}}\thishybrid[#1]}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\newtheoremstyle{hybrid}% name of the style to be used
  {1em}% measure of space to leave above the theorem. E.g.: 3pt
  {1em}% measure of space to leave below the theorem. E.g.: 3pt
  {}% name of font to use in the body of the theorem
  {0pt}% measure of space to indent
  {\bfseries}% name of head font
  {}% punctuation between head and body
  {0pt}% space after theorem head; " " = normal interword space
  {\stepcounter{realprevhybrid}\stepcounter{prevhybrid}\stepcounter{hybrids}\refstepcounter{realhybrids}\thmname{#1} \thishybrid[#3]. \label{hybauto:\arabic{realhybrids}}}
\theoremstyle{hybrid}
\newtheorem*{hybrid}{Hybrid}

\newcommand{\hyb}{\ensuremath{\mathcal{H}}\xspace}
\newcommandx{\thishybrid}[1][1={}]{\ensuremath{\hyperref[hybauto:\arabic{realhybrids}]{\ifthenelse{\equal{#1}{}}{\hyb_{\arabic{hybrids}}}{#1}}}\xspace}
\newcommandx{\thathybrid}[2][2={}]{\ensuremath{\hyperref[hybauto:\getrefnumber{real#1}]{\ifthenelse{\equal{#2}{}}{\hyb_{\getrefnumber{#1}}}{#2}}}\xspace}
\newcommandx{\firsthybrid}[1][1={}]{\ensuremath{\hyperref[hybauto:\arabic{realfirsthybrid}]{\ifthenelse{\equal{#1}{}}{\hyb_0}}{#1}}\xspace}
\newcommandx{\prevhybrid}[1][1={}]{\ensuremath{\hyperref[hybauto:\arabic{realprevhybrid}]{\ifthenelse{\equal{#1}{}}{\hyb_{\arabic{prevhybrid}}}{#1}}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheoremstyle{protosec}% name of the style to be used
  {0pt}% measure of space to leave above the theorem. E.g.: 3pt
  {0pt}% measure of space to leave below the theorem. E.g.: 3pt
  {}% name of font to use in the body of the theorem
  {0pt}% measure of space to indent
  {\bfseries}% name of head font
  {:}% punctuation between head and body
  { }% space after theorem head; " " = normal interword space
  {#3}
\theoremstyle{protosec}
\newtheorem*{protosec}{}

\newtheoremstyle{algorithm}% name of the style to be used
  {\topsep}% measure of space to leave above the theorem. E.g.: 3pt
  {0pt}% measure of space to leave below the theorem. E.g.: 3pt
  {}% name of font to use in the body of the theorem
  {0pt}% measure of space to indent
  {\bfseries}% name of head font
  { }% punctuation between head and body
  { }% space after theorem head; " " = normal interword space
  {\strut\iffalse\hspace*{-0.25em}\rlap{\colorbox{white}{\thmname{#1}\thmnumber{ #2.}\thmnote{ #3}~}}\fi}

\theoremstyle{algorithm}

\newaliascnt{intalg}{boxctr}
\newtheorem{intalg}[intalg]{Algorithm}
\aliascntresetthe{intalg}

\newaliascnt{intprog}{boxctr}
\newtheorem{intprog}[intprog]{Program}
\aliascntresetthe{intprog}

\newaliascnt{intexpt}{boxctr}
\newtheorem{intexpt}[intexpt]{Experiment}
\aliascntresetthe{intexpt}

\newaliascnt{intfunc}{boxctr}
\newtheorem{intfunc}[intfunc]{Functionality}
\aliascntresetthe{intfunc}

\newaliascnt{intprot}{boxctr}
\newtheorem{intprot}[intprot]{Protocol}
\aliascntresetthe{intprot}

\newaliascnt{intsimu}{boxctr}
\newtheorem{intsimu}[intsimu]{Simulator}
\aliascntresetthe{intsimu}

\newaliascnt{intgame}{boxctr}
\newtheorem{intgame}[intgame]{Game}
\aliascntresetthe{intgame}

\makeatletter
\newenvironment{intrecalg}[2]
  {\count@\c@intalg
   \global\c@intalg#1 %
    \global\advance\c@intalg\m@ne
   \intalg[#2]}
  {\endintalg
   \global\c@intalg\count@}
\makeatother

\mdfdefinestyle{barstyle}{
  hidealllines=false,
  innerleftmargin=0.5em,
  innerrightmargin=1em,
  innertopmargin=0.5em,
  innerbottommargin=0.5em,
  skipabove=0.2em,
  skipbelow=0.35em,
}

\mdfdefinestyle{barstylewtitle}{
  rightline=false,
  bottomline=false,
  topline=false,
  innerleftmargin=1em,
  innerrightmargin=0em,
  innertopmargin=0.8em,
  innerbottommargin=0em,
  skipabove=0pt,
  skipbelow=0.5em,
  frametitleaboveskip=0pt,
  frametitlebackgroundcolor=white,
  frametitlealignment=\raggedright
}

\mdfdefinestyle{boxstylewtitle}{
  hidealllines=false,
  innerleftmargin=1em,
  innerrightmargin=1em,
  innertopmargin=0.8em,
  innerbottommargin=1em,
  skipabove=0pt,
  skipbelow=0.5em,
  frametitleaboveskip=0pt,
  frametitlebackgroundcolor=white,
  frametitlealignment=\raggedright
}

\newenvironment{algorithm}[1][]{\Needspace{4\baselineskip}\par\intalg[#1]~\vspace{-1em}\begin{mdframed}[style=boxstylewtitle,frametitle={\hspace*{-1.2em}\smash{\raisebox{-0.25em}{\rlap{\colorbox{white}{Algorithm \thesection.\arabic{intalg}. #1\strut~}}}}}]}{\end{mdframed}\endintalg}
\newenvironment{program}[1][]{\Needspace{4\baselineskip}\par\intprog[#1]~\vspace{-1em}\begin{mdframed}[style=boxstylewtitle,frametitle={\hspace*{-1.2em}\smash{\raisebox{-0.25em}{\rlap{\colorbox{white}{Program \thesection.\arabic{intprog}. #1\strut~}}}}}]}{\end{mdframed}\endintprog}
\newenvironment{experiment}[1][]{\Needspace{4\baselineskip}\par\intexpt[#1]~\vspace{-1em}\begin{mdframed}[style=boxstylewtitle,frametitle={\hspace*{-1.2em}\smash{\raisebox{-0.25em}{\rlap{\colorbox{white}{Experiment \thesection.\arabic{intexpt}. #1\strut~}}}}}]}{\end{mdframed}\endintexpt}
\newenvironment{functionality}[1][]{\Needspace{4\baselineskip}\par\intfunc[#1]~\vspace{-1em}\begin{mdframed}[style=boxstylewtitle,frametitle={\hspace*{-1.2em}\smash{\raisebox{-0.25em}{\rlap{\colorbox{white}{Functionality \thesection.\arabic{intfunc}. #1\strut~}}}}}]}{\end{mdframed}\endintfunc}
\newenvironment{protocol}[1][]{\Needspace{4\baselineskip}\par\intprot[#1]~\vspace{-1em}\begin{mdframed}[style=boxstylewtitle,frametitle={\hspace*{-1.2em}\smash{\raisebox{-0.25em}{\rlap{\colorbox{white}{Construction \thesection.\arabic{intprot}. #1\strut~}}}}}]}{\end{mdframed}\endintprot}
\newenvironment{simulator}[1][]{\Needspace{4\baselineskip}\par\intsimu[#1]~\vspace{-1em}\begin{mdframed}[style=boxstylewtitle,frametitle={\hspace*{-1.2em}\smash{\raisebox{-0.25em}{\rlap{\colorbox{white}{Simulator \thesection.\arabic{intsimu}. #1\strut~}}}}}]}{\end{mdframed}\endintsimu}
\newenvironment{gamebox}[1][]{\Needspace{4\baselineskip}\par\intgame[#1]~\vspace{-1em}\begin{mdframed}[style=boxstylewtitle,frametitle={\hspace*{-1.2em}\smash{\raisebox{-0.25em}{\rlap{\colorbox{white}{Game \thesection.\arabic{intgame}. #1\strut~}}}}}]}{\end{mdframed}\endintgame}

%\renewenvironment{definition}[1][]{\Needspace{4\baselineskip}\par\intdef[#1]~\vspace{-1em}\begin{mdframed}[style=boxstylewtitle,frametitle={\hspace*{-1.2em}\smash{\raisebox{-0.25em}{\rlap{\colorbox{white}{Definition \thesection.\arabic{intdef}. #1\strut~}}}}}]}{\end{mdframed}\endintdef}

\ifdefined\isllncs{
    \renewcommand\theboxctr{\thesection.\arabic{boxctr}}
    \makeatletter
}\fi

\newenvironment{proofsketch}{%
\renewcommand{\proofname}{Proof Sketch}\proof}{\endproof}


\makeatletter
\newcommand{\subalign}[1]{%
  \vcenter{%
    \Let@ \restore@math@cr \default@tag
    \baselineskip\fontdimen10 \scriptfont\tw@
    \advance\baselineskip\fontdimen12 \scriptfont\tw@
    \lineskip\thr@@\fontdimen8 \scriptfont\thr@@
    \lineskiplimit\lineskip
    \ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\hfil\crcr
      #1\crcr
    }%
  }%
}
\makeatother 

